Parallel numerical method for nonlocal-in-time Schr\"odinger equation

We present a new parallel numerical method for solving the non-stationary Schr\"odinger equation with linear nonlocal condition and time-dependent potential which does not commute with the stationary part of the Hamiltonian. The given problem is discretized in-time using a polynomial-based collocation scheme. We establish the conditions on the existence of solution to the discretized problem, estimate the accuracy of the discretized solution and propose the method how this solution can be approximately found in an efficient parallel manner.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	//
Abstract and Keywords	JCSMD-Latex-Template-2column.tex	/^ \\subsubsection{Abstract and Keywords}$/;"	b	subsection:Preparation of Manuscripts""Organization of the Manuscript
Acceptance Criteria	JCSMD-Latex-Template-2column.tex	/^\\section{Acceptance Criteria}$/;"	s
Acknowledgements	JCSMD-Latex-Template-2column.tex	/^\\label{Acknowledgements}$/;"	l
Acknowledgments	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Acknowledgments}$/;"	b	subsection:Preparation of Manuscripts""Organization of the Manuscript
Author Related Work and Electronic Data Files	JCSMD-Latex-Template-2column.tex	/^\\subsection{Author Related Work and Electronic Data Files}$/;"	u	section:Manuscript Submission and Peer Review Process
Benefits to the Authors and Offprints	JCSMD-Latex-Template-2column.tex	/^\\section{Benefits to the Authors and Offprints}$/;"	s
Conclusions	JCSMD-Latex-Template-2column.tex	/^\\label{Conclusions}$/;"	l
Conclusions	JCSMD-Latex-Template-2column.tex	/^\\section{Conclusions}$/;"	s
Conclusions	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Conclusions}$/;"	b	subsection:Preparation of Manuscripts""Organization of the Manuscript
Conclusions	sytnyk_2018.tex	/^	\\section*{Conclusions}\\label{sec:conclussions}$/;"	s
ContSolRepSE	sytnyk_2018.tex	/^		\\begin{equation}\\label{ContSolRepSE}$/;"	l
Copyright Transfer Agreement	JCSMD-Latex-Template-2column.tex	/^ \\subsection{Copyright Transfer Agreement}$/;"	u	section:Preparation of Manuscripts
Cover Art and Supplemental Material	JCSMD-Latex-Template-2column.tex	/^ \\subsection{Cover Art and Supplemental Material}$/;"	u	section:Preparation of Manuscripts
Cover Letter	JCSMD-Latex-Template-2column.tex	/^\\subsection{Cover Letter}$/;"	u	section:Manuscript Submission and Peer Review Process
Decision Letter	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Decision Letter}$/;"	b	subsection:Manuscript Submission and Peer Review Process""Peer Review Process
Discretization scheme	sytnyk_2018.tex	/^\\section{Discretization scheme}\\label{sec:discratization}$/;"	s
Figures and Tables	JCSMD-Latex-Template-2column.tex	/^\\subsection{Figures and Tables}$/;"	u	section:Preparation of Manuscripts
Final proofreading	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Final proofreading}$/;"	b	subsection:Manuscript Submission and Peer Review Process""Peer Review Process
Formatting and Readability	JCSMD-Latex-Template-2column.tex	/^ \\subsection{Formatting and Readability}$/;"	u	section:Preparation of Manuscripts
General remarks	JCSMD-Latex-Template-2column.tex	/^\\subsection{General remarks}$/;"	u	section:Preparation of Manuscripts
Implementation	sytnyk_2018.tex	/^	\\section{Implementation}\\label{sec:impl_ex}$/;"	s
Introduction	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Introduction}$/;"	b	subsection:Preparation of Manuscripts""Organization of the Manuscript
Introduction	sytnyk_2018.tex	/^\\section*{Introduction}$/;"	s
JCSMD Aims and Scope	JCSMD-Latex-Template-2column.tex	/^\\section{JCSMD Aims and Scope}$/;"	s
JCSMD Submission Checklist	JCSMD-Latex-Template-2column.tex	/^\\subsection{JCSMD Submission Checklist}$/;"	u	section:Manuscript Submission and Peer Review Process
Main Part of the Article	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Main Part of the Article}$/;"	b	subsection:Preparation of Manuscripts""Organization of the Manuscript
Manuscript Submission and Peer Review Process	JCSMD-Latex-Template-2column.tex	/^\\section{Manuscript Submission and Peer Review Process}$/;"	s
Mission of the Journal	JCSMD-Latex-Template-2column.tex	/^\\label{Mission of the Journal}$/;"	l
Notation  Mathematical Material  and Nomenclature	JCSMD-Latex-Template-2column.tex	/^ \\subsection{Notation, Mathematical Material, and Nomenclature}$/;"	u	section:Preparation of Manuscripts
Numerical method for propagator approximation	sytnyk_2018.tex	/^\\section{Numerical method for propagator approximation}\\label{sec:op_func_approx}	$/;"	s
Organization of the Manuscript	JCSMD-Latex-Template-2column.tex	/^ \\subsection{Organization of the Manuscript}$/;"	u	section:Preparation of Manuscripts
Other Issues	JCSMD-Latex-Template-2column.tex	/^ \\subsubsection{Other Issues}$/;"	b	subsection:Manuscript Submission and Peer Review Process""Peer Review Process
ParHomSolSE	sytnyk_2018.tex	/^	\\begin{equation}\\label{ParHomSolSE}$/;"	l
Peer Review Process	JCSMD-Latex-Template-2column.tex	/^\\subsection{Peer Review Process}$/;"	u	section:Manuscript Submission and Peer Review Process
Permissions	JCSMD-Latex-Template-2column.tex	/^\\subsection{Permissions}$/;"	u	section:Manuscript Submission and Peer Review Process
Preparation of Manuscripts	JCSMD-Latex-Template-2column.tex	/^\\section{Preparation of Manuscripts}$/;"	s
References and Footnotes	JCSMD-Latex-Template-2column.tex	/^ \\subsection{References and Footnotes}$/;"	u	section:Preparation of Manuscripts
Resubmission	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Resubmission}$/;"	b	subsection:Manuscript Submission and Peer Review Process""Peer Review Process
Table:param:one	JCSMD-Latex-Template-2column.tex	/^  \\label{Table:param:one}$/;"	l
Title	JCSMD-Latex-Template-2column.tex	/^\\subsubsection{Title}$/;"	b	subsection:Preparation of Manuscripts""Organization of the Manuscript
alg:o_f	sytnyk_2018.tex	/^	\\label{alg:o_f}$/;"	l
alg:sol_it_sys	sytnyk_2018.tex	/^	\\label{alg:sol_it_sys}$/;"	l
code:res_eqs	sytnyk_2018.tex	/^		\\FOR{$m=-n$ \\TO $n$}\\label{code:res_eqs}$/;"	l
eq:Alg_dec_strip	sytnyk_2018.tex	/^		\\begin{equation}\\label{eq:Alg_dec_strip}$/;"	l
eq:ApproxHomSolSE	sytnyk_2018.tex	/^	\\begin{equation}\\label{eq:ApproxHomSolSE}$/;"	l
eq:ApproxInhomSolSE	sytnyk_2018.tex	/^	\\begin{equation}\\label{eq:ApproxInhomSolSE}$/;"	l
eq:C_est	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:C_est}$/;"	l
eq:EN	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:EN}$/;"	l
eq:NCPPropSolRepSE	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:NCPPropSolRepSE}$/;"	l
eq:NCPSchrodEqt	sytnyk_2018.tex	/^{i}\\frac{\\partial\\Psi}{\\partial t}-(H+v(t))\\Psi= 0, \\label{eq:NCPSchrodEqt}\\\\$/;"	l
eq:NCP_transf	sytnyk_2018.tex	/^{i}\\frac{\\partial\\psi}{\\partial s}-H\\psi = iV(s)\\psi, \\label{eq:NCP_transf}\\\\$/;"	l
eq:NCPnonloc_cond	sytnyk_2018.tex	/^\\label{eq:NCPnonloc_cond} %\\quad \\alpha_k \\in \\mathrm{C}, \\ t_k \\in (0, T].$/;"	l
eq:NCPnonloc_cond_transf	sytnyk_2018.tex	/^\\label{eq:NCPnonloc_cond_transf} %\\quad \\alpha_k \\in \\mathrm{C}, \\ t_k \\in (0, T].$/;"	l
eq:ResHalfStrip	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:ResHalfStrip}$/;"	l
eq:S1_inv	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:S1_inv}$/;"	l
eq:SC_est	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:SC_est}$/;"	l
eq:SF_el_calc_func	sytnyk_2018.tex	/^	\\begin{equation*}\\label{eq:SF_el_calc_func}$/;"	l
eq:S_est	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:S_est}$/;"	l
eq:S_inv_repr	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:S_inv_repr}$/;"	l
eq:SchrodEqt	sytnyk_2018.tex	/^\\begin{equation} \\label{eq:SchrodEqt}$/;"	l
eq:Sinv_Ck	sytnyk_2018.tex	/^		C^\\Upsilon_k &= \\suml_{j=0}^N g(s_k,H,j)\\Phi_j,\\label{eq:Sinv_Ck}\\\\$/;"	l
eq:Sinv_Ck_g	sytnyk_2018.tex	/^		g(s,z,j) &= \\suml_{l=1}^{N} f(s,z,l) \\int\\limits_{s_{l-1}}^{s_l} e^{iz t}V(t)L_{j}(t)dt .\\/;"	l
eq:SpHalfStrip	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:SpHalfStrip}$/;"	l
eq:V_Lip	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:V_Lip}$/;"	l
eq:best_approx	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:best_approx}$/;"	l
eq:err_est_no_N1	sytnyk_2018.tex	/^		\\begin{equation}\\label{eq:err_est_no_N1}$/;"	l
eq:h_no_N1	sytnyk_2018.tex	/^		\\begin{equation*}\\label{eq:h_no_N1}$/;"	l
eq:initial_state_NCNS	sytnyk_2018.tex	/^ 	\\begin{equation}\\label{eq:initial_state_NCNS}$/;"	l
eq:int_cont	sytnyk_2018.tex	/^	\\begin{equation}\\label{eq:int_cont}$/;"	l
eq:int_repr_seq_pol	sytnyk_2018.tex	/^\\label{eq:int_repr_seq_pol}$/;"	l
eq:iter_solution	sytnyk_2018.tex	/^		\\begin{equation} \\label{eq:iter_solution}$/;"	l
eq:lagrange_pol	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:lagrange_pol}$/;"	l
eq:mat_norm_X	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:mat_norm_X}$/;"	l
eq:matrix_sys	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:matrix_sys}$/;"	l
eq:matrix_sys_bound	sytnyk_2018.tex	/^		\\begin{equation}\\label{eq:matrix_sys_bound}$/;"	l
eq:nc_transf_pol	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:nc_transf_pol}$/;"	l
eq:prop_int_prop	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:prop_int_prop}$/;"	l
eq:res_eq	sytnyk_2018.tex	/^	\\begin{equation}\\label{eq:res_eq}$/;"	l
eq:tau_max	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:tau_max}$/;"	l
eq:var_transform	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:var_transform}$/;"	l
eq:vec_norm_X	sytnyk_2018.tex	/^\\begin{equation}\\label{eq:vec_norm_X}$/;"	l
eq:zerosExpI	sytnyk_2018.tex	/^ 	\\label{eq:zerosExpI}$/;"	l
estamate:hopt	JCSMD-Latex-Template-2column.tex	/^  \\label{estamate:hopt}$/;"	l
fig:env2stripe	sytnyk_2018.tex	/^	\\label{fig:env2stripe}$/;"	l
figb	JCSMD-Latex-Template-2column.tex	/^\\caption{\\label{figb}(Color online) Effect of piezoelectric potential on the two vertically st/;"	l
normalsize Acknowledgments	JCSMD-Latex-Template-2column.tex	/^\\section*{\\normalsize Acknowledgments}$/;"	s
normalsize References	JCSMD-Latex-Template-2column.tex	/^\\section*{\\normalsize References}$/;"	s
reprDunford	sytnyk_2018.tex	/^ \\label{reprDunford}$/;"	l
sec:conclussions	sytnyk_2018.tex	/^	\\section*{Conclusions}\\label{sec:conclussions}$/;"	l
sec:discratization	sytnyk_2018.tex	/^\\section{Discretization scheme}\\label{sec:discratization}$/;"	l
sec:impl_ex	sytnyk_2018.tex	/^	\\section{Implementation}\\label{sec:impl_ex}$/;"	l
sec:op_func_approx	sytnyk_2018.tex	/^\\section{Numerical method for propagator approximation}\\label{sec:op_func_approx}	$/;"	l
thm:NCNS_exist_mild	sytnyk_2018.tex	/^ \\begin{thm}[\\cite{SytnykMelnik2018}]\\label{thm:NCNS_exist_mild}$/;"	l
thm:SQ_alg_decay_strip	sytnyk_2018.tex	/^	\\begin{thm}[\\cite{schrod_num_Sytnyk2017}]\\label{thm:SQ_alg_decay_strip}$/;"	l
thm:S_inv	sytnyk_2018.tex	/^\\begin{lemma}\\label{thm:S_inv}$/;"	l
thm:main	sytnyk_2018.tex	/^\\begin{thm}\\label{thm:main}$/;"	l
thm:matrix_est	sytnyk_2018.tex	/^\\begin{lemma}\\label{thm:matrix_est}$/;"	l

